Seq2Time: Sequential Knowledge Transfer for Video LLM Temporal Grounding

Temporal awareness is essential for video large language models (LLMs) to understand and reason about events within long videos, enabling applications like dense video captioning and temporal video grounding in a unified system. However, the scarcity of long videos with detailed captions and precise temporal annotations limits their temporal awareness. In this paper, we propose Seq2Time, a data-oriented training paradigm that leverages sequences of images and short video clips to enhance temporal awareness in long videos. By converting sequence positions into temporal annotations, we transform large-scale image and clip captioning datasets into sequences that mimic the temporal structure of long videos, enabling self-supervised training with abundant time-sensitive data. To enable sequence-to-time knowledge transfer, we introduce a novel time representation that unifies positional information across image sequences, clip sequences, and long videos. Experiments demonstrate the effectiveness of our method, achieving a 27.6% improvement in F1 score and 44.8% in CIDEr on the YouCook2 benchmark and a 14.7% increase in recall on the Charades-STA benchmark compared to the baseline.

==> sec/5_discussion.tex <==
\section{Discussion}

\begin{figure*}[ht]
\centering
% \vspace{-0.2cm}
\scalebox{1}{\includegraphics[width=1\textwidth]{figures/qualitative_results.pdf}}
\caption{Qualitative examples of \method on TimeChat. IS means image sequence data, CS means clip sequence data and MC means more video captions. The \textcolor{red}{\textbf{red text}} indicates repetitive patterns in the output captions and the \textcolor{brown}{\textbf{brown text}} indicates false prediction in timestamps and events. It can be noted that adding image sequence data could reduce the repetitive patterns for TimeChat to a large degree. Although there are wrong recognitions (\eg, recognizing the pan as an oven), training with \method provides more accurate descriptions and precise timestamp predictions.} 
\label{fig:example}
% \vspace{-12pt}
\end{figure*}

\subsection{Dataset Effect}
To analyze how different data components influence temporal understanding in video LLMs, we conduct comprehensive ablation studies on TimeChat, as shown in Table~\ref{tab:dataset_ablation}. The removal of clip sequence data leads to performance drops in both dense video captioning and temporal grounding tasks, demonstrating its importance in the training pipeline.

Interestingly, incorporating additional video captions from ShareGPT4video~\cite{chen2024sharegpt4video} shows unexpected effects: while it doesn't significantly improve captioning quality, it substantially enhances temporal perception, yielding a 19.5\% improvement in YouCook2's F1 score and 7.3\% in Charades-STA's R@1(IoU=0.5). We hypothesize that exposure to more captions improves the model's ability to understand long-form video content, leading to better event boundary detection.

The impact of image sequence data (IS) is particularly striking, especially in text generation quality. The CIDEr score shows a remarkable 48.3\% improvement over the baseline, providing strong evidence that temporal understanding can be effectively learned from static image sequences. To further validate this finding, we tested our image sequence data on Video-LLaMA, a general video LLM without prior temporal training. As shown in Table~\ref{tab:is_on_dvc}, while the base model struggles with temporal events (F1 score of 0.2), adding image sequence training improves this to 3.3, demonstrating initial temporal awareness. Notably, this improvement occurs even without our unified relative position tokens, using only free-form language for index representation. This confirms that sequential knowledge can be effectively transferred across different data modalities.

In addition to dense video captioning performance with common metrics, we also evaluate the impact of different training datasets on the number of predicted events per video and the lexical richness of the generated captions, as shown in Table~\ref{tab:ttr}. While adding new training data does not significantly alter the number of predicted events ($n_{\text{pred}}$), it does have a noticeable effect on the lexical richness of the captions. To assess text richness, we measure the average caption length ($L_{\text{avg}}$) and the Type-Token Ratio (TTR)~\cite{malvern2004lexical}, which quantifies lexical diversity. As indicated in the results, incorporating additional training data consistently enhances the richness and diversity of the generated captions, resulting in more descriptive and meaningful outputs. More details can be found in ~\textbf{Supplementary}.

\begin{table}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
method           & $n_{\text{pred}}$ & $L_{\text{avg}}$ & TTR \\ 
\midrule
TimeChat         & 11.04   & 6.81         & 0.268 \\ 
+IS              & 8.44    & 8.19         & 0.411 \\ 
+IS+MC           & 11.53   & 8.74         & 0.384 \\ 
+\method         & 8.94    & 11.5         & 0.396 \\ 
\bottomrule
\end{tabular}
\caption{Impact of different data on dense video captioning. $n_{\text{pred}}$ means the average event number in the prediction, $L_{\text{avg}}$ means the average length for each caption and TTR means Type-Token Ratio.}
\label{tab:ttr}
\end{table}


% This indicates learning the image-captioning correspondence from a long image sequence could indeed enhance the time-sensitivity of video LLMs.

\subsection{Image-based Pretext Tasks}
% In this section, we experimentally evaluate the individual effect of each pretext task in our image sequence data. In the experiments, to remove the effect of the number of training samples, we fix the total number of image sequence data but only change the existence of a specific pretext task. For instance, in the second row of Table~\ref{tab:pretext_task_ablation}, the adjacent location reasoning is removed during training, and the sampling number of the other two pretext tasks increases to 150K each. Comparing the first two rows, we can observe a clear drop in CIDEr, which indicates the effectiveness of indexed image captioning (IIC) on text generation. After removing the image index grounding (IIG), we can observe a general performance degradation on both benchmarks. This demonstrates that IIG plays a more important role compared with IIC. Additionally, comparing the third row with the last row, which is the TimeChat baseline results, we can also obtain another interesting result that only increasing the number of training data cannot guarantee a better performance, the data composition is a more critical factor. For the adjacent location reasoning (ALR),  comparing the 4-th row with the 1-st row, we can observe that ALR has a significant impact on the text generation performance, after removing this task, the CIDEr drop 37.2\% while SODA\_c drops 40\%. Moreover, comparing the last two rows, we can also see the the sequence localization improvement brought by IIC and IIG, \ie, a 13.4\% improvement after adding 300K IIC and IIG data.

We analyze the contribution of each pretext task while controlling for training data volume by maintaining a fixed total amount of image sequence data. Table~\ref{tab:pretext_task_ablation} shows our systematic evaluation where omitted tasks are compensated by increasing the sampling of remaining tasks (\eg, when removing ALR, IIC and IIG samples increase to 150K each).

Our analysis reveals distinct roles for each task. Indexed Image Captioning (IIC) primarily enhances text generation quality, as evidenced by the significant CIDEr score drop when IIC is absent. Image Index Grounding (IIG) proves crucial for overall temporal understanding, with its removal causing performance degradation across both benchmarks, suggesting a stronger impact than IIC. Adjacent Location Reasoning (ALR) substantially influences text generation capabilities—its removal leads to a 37.2\% decrease in CIDEr and 40\% in SODA\_c scores.

Importantly, comparing the baseline TimeChat with variants using only IIC and IIG shows that performance improvements depend more on task diversity than data volume—adding 300K samples of just IIC and IIG data yields only a 13.4\% improvement. This underscores the importance of our complementary task design in developing robust temporal understanding capabilities.


\subsection{Dataset Scaling}
To investigate the scaling properties of Seq2Time, we conduct experiments with varying proportions (5\% and 20\%) of our image sequence and clip sequence data using TimeChat as the baseline model. As shown in Table~\ref{tab:dataset_scaling}, even with just 5\% of our data, we observe notable improvements in dense video captioning performance, particularly in the CIDEr metric which measures text generation quality. The performance scales positively with data volume, showing consistent improvements across both dense video captioning and temporal video grounding tasks as we increase the proportion of \method data. Detailed scaling analysis and additional results are provided in the \textbf{Supplementary}.

\subsection{Results Visualization}
% To qualitatively demonstrate the effectiveness of \method, we present a comparison based on TimeChat in Figure~\ref{fig:example}. The original TimeChat often generates redundant text, highlighted by the red text in the figure, a problem that is significantly mitigated after training with \method. This phenomenon may result from the limited captioning data in TimeIT; however, \method benefits from high-quality captioning data available in both image and clip sequence datasets. Besides, \method could also address the hullucination problem in dense video captioning task. In the second example in Figure~\ref{fig:example}, the original TimeChat wrongly response with "takes a spoon of water from the sink" in the beginning segments, in comparison, after training with \method, the model tends to output correct description that "put a pot of water on the stove".
% Additionally, the output from \method provides more detailed object descriptions as illustrated in the first example. Nevertheless, there are still some failure response, for instance, in the third example, the "tofu" is mistakenly recognized as "tomato". This could be potentially solved with more advanced visual encoder in future study.

To qualitatively demonstrate the effectiveness of Seq2Time, we analyze different model variants in Figure~\ref{fig:example}. The baseline TimeChat tends to generate repetitive patterns—for instance, repeatedly mentioning \textit{knead the dough} throughout the video when this action only occurs between 120s and 200s. This phenomenon is consistent with the low TTR of TimeChat in Table~\ref{tab:ttr}. This limitation likely stems from insufficient captioning data in TimeIT. However, our \method, leveraging rich captions from both image and clip sequence datasets, significantly improves temporal and descriptive accuracy.

The addition of image sequence data (IS) yields two key improvements. First, it eliminates repetitive captioning patterns. Second, it enhances temporal precision—for example, the model accurately localizes the event \textit{water and salt are added into the bowl} to 34.8-76.4 seconds, closely matching the ground truth of 48-79 seconds. This improvement aligns with our quantitative findings in Table~\ref{tab:dataset_ablation}, where image sequence data substantially improves the CIDEr score.

In the full version (blue patch), the model demonstrates even more precise temporal and descriptive capabilities. For instance, it correctly identifies and localizes the event \textit{the mixture is then put in a bowl and water is poured over it} to 95.2-123.2 seconds, matching the ground truth event \textit{add salt, plain yogurt, and water and mix to form a dough} (80-133 seconds). While some fine-grained object recognition challenges remain, temporal localization is accurate.

\noindent \textbf{Failure Case Analysis}\quad Despite overall improvements, we observe several types of prediction errors. With only image sequence data, object recognition errors occur—for example, misidentifying a blender as hands during dough mixing. Adding more video caption data (+IS+MC) reduces but doesn't eliminate all repetitive patterns, and sometimes confuses similar objects (\eg, identifying dough as bread). Even in the full version, we notice object recognition errors (pan mistaken for oven) and hallucinated events (\eg, \textit{cut into different shapes}). These issues primarily stem from visual recognition limitations and suggest that incorporating more advanced visual encoders could further improve model performance.

% The original TimeChat often generates redundant text, highlighted by the red text in the figure, a problem that is significantly mitigated after training with \method. This phenomenon may result from the limited captioning data in TimeIT; however, \method benefits from high-quality captioning data available in both image and clip sequence datasets. Moreover, \method also addresses the hallucination problem in dense video captioning tasks. In the second example in Figure~\ref{fig:example}, the original TimeChat incorrectly responds with "takes a spoon of water from the sink" in the beginning segments. In comparison, after training with \method, the model outputs the correct description, "puts a pot of water on the stove." 
% Additionally, the output from \method provides more detailed object descriptions, as illustrated in the first example. Nevertheless, some errors persist; for instance, in the third example, "tofu" is mistakenly recognized as "tomato." 

